Measuring algorithmic interpretability: A human-learning-based framework and the corresponding cognitive complexity score

Algorithmic interpretability is necessary to build trust, ensure fairness, and track accountability. However, there is no existing formal measurement method for algorithmic interpretability. In this work, we build upon programming language theory and cognitive load theory to develop a framework for measuring algorithmic interpretability. The proposed measurement framework reflects the process of a human learning an algorithm. We show that the measurement framework and the resulting cognitive complexity score have the following desirable properties - universality, computability, uniqueness, and monotonicity. We illustrate the measurement framework through a toy example, describe the framework and its conceptual underpinnings, and demonstrate the benefits of the framework, in particular for managers considering tradeoffs when selecting algorithms.

==> broaderimpact.tex <==
%\subsection{Broader Impact}


\textit{A new dimension for algorithm comparison.}
This framework is meant to complement existing measures for quantify algorithms, such as runtime complexity.
Quantifying interpretability provides one more dimension in which algorithms can be compared to one another.
An algorithm may have a higher runtime complexity, but is more interpretable.
This tradeoff can now be quantified and analyzed on a case-by-case basis according to user requirements.
%Scoring algorithmic interpretability can also be used to move research in the field forward.
%Different methods and tools for making existing algorithms more interpretable 
New algorithms can now be scored based on interpretability and compared against one another, according to specific types of users (high or low algorithmic literacy). 

\textit{A mechanism for improving user understanding.}
A key feature of this framework is that it is user-specific. 
A representation depends on the algorithmic literacy of the user.
For researchers, understanding the user when generating representations comes with two key benefits.
First, the researcher can provide a representation that is appropriate given the user's algorithmic literacy level, removing confusion and frustration.
Second, because we associate algorithmic literacy levels with specific operations, users with low algorithmic literacy can be provided with an appropriate representation, as well as a list of operations associated with a high algorithmic literacy representation. 
This provides a specific learning opportunity for the users. If they can understand those operations, then they can understand a more compact, higher-level representation of the algorithm.
For our RecSys example, if a low algorithmic literacy user wants to better understand user-user KNN, he or she would have to learn how to calculate L2 norms and dot products.

%Quantifying algorithmic interpretability is a different dimension than post-hoc explainability.
%Post-hoc explainability methods typically try to make existing algorithms more interpretable via explanations of specific cases.
%In this work we argue that all algorithms are interpretable to a degree, and that interpretability can be quantified. 

\textit{Appropriateness for complex models.}
The framework presented is general enough to cover even extremely complex algorithms.
While their representations will be more complex than those in the examples presented here, even complex algorithms can be broken down into operations and contexts and represented as such. 
%We argue that there is no such thing as a ``non-interpretable'' algorithm.
With the proposed framework even complex algorithms can be represented and their interpretability can be scored.
For a long time it has been assumed that such algorithms are less interpretable (or not interpretable at all) compared to simpler algorithms.
Now such comparisons can be quantified and tested. 

\textit{Contributions to research. } 
%The proposed research framework makes the following contributions to the existing literature.
To the best of our knowledge, this is the first work to quantify algorithmic interpretability. 
The interpretability score can be used to evaluate tradeoffs between different performance dimensions for algorithms.
%Analogous to the ``big-O'' notation for runtime complexity, the generated algorithmic interpretability score from our research framework measures another important dimension of algorithms -- interpretability. 
%There are critical differences between runtime complexity and interpretability: runtime complexity is machine-oriented and interpretability is human-oriented.
%For example, multiple loops through a data set affect runtime but do not change the difficulty level of understanding the algorithm.
%On the other hand, it is easy for computers to keep track of different contexts but challenging for human to do so.
Our proposed framework explicitly captures both operations and contexts from the users' perspective to measure this new dimension of algorithmic performance -- interpretability.
Finally we introduce two enhanced graphical representations of algorithms (context-aware directed graph and context-aware reverse-path tree) and two corresponding scoring methods (in-neighbor aggregation and reverse-path tree) to generate a unique score of algorithmic interpretability. 
These presentations and scoring methods have desirable properties (equivalence, uniqueness, and order preserving) and can be applied to all algorithms.

\textit{Contributions to practice. } The proposed framework can potentially benefit a variety of stakeholders:
	\textit{Software developers} can provide various interpretable representations of their newly developed algorithms as documentation for downstream stakeholders.
	\textit{Researchers} can evaluate new algorithms in terms of interpretability in a quantifiable way.
	This provides a new performance dimension for future work when comparing against existing methods.
	\textit{Firms} implementing a new algorithmic process can assess the tradeoffs associated with more- or less-interpretable models.
	\textit{Users} can request an algorithmic representation at an appropriate level for them, and also compare apps, websites, etc. in terms of how interpretable their algorithmic processes are. 
	%Interpretability can also affect how much a user trusts a particular firm.

%\begin{comment} 
\textit{Ethical considerations. }
One risk with the proposed framework is that quantifying interpretability devolves into just another metric to optimize.
Firms or developers may try to ``optimize'' interpretability by cutting corners on algorithms or obfuscating steps to reduce the interpretability graph size.
Such behaviors diminish the expected benefits of measuring interpretability, and should be avoided.
That said, such risks are present for any such measurement, and safeguards that currently exist can also be applied here.
Peer-review of interpretability metrics as a regular part of new algorithm development will ensure that claims made about the interpretability of an algorithm are validated.
Regulatory bodies can check reported interpretability metrics via audits.
%\end{comment}


==> old_introduction.tex <==
% old intro below

Outline:
\begin{itemize}
    \item Algorithms are widespread and important.
    \item Algorithmic interpretability is important: how it is related to trust, FATE
    \item Measuring algorithmic interpretability is important: measuring algorithmic interpretability is the foundation for the evaluation of XAI methods.
    \item Existing work and research gap
    \item Our solution -- framework and score
    \item Our contribution
\end{itemize}



%Precise measurements for fairness, bias, and accountability are hard to define, so as a proxy researchers have turned to algorithm interpretability \cite{doshi-velezRigorousScienceInterpretable2017,lipton2018mythos}.
Regulators want to assess models for potential biases.\footnote{https://www.ftc.gov/news-events/blogs/business-blog/2021/04/aiming-truth-fairness-equity-your-companys-use-ai}\footnote{https://digital-strategy.ec.europa.eu/en/library/proposal-regulation-laying-down-harmonised-rules-artificial-intelligence-artificial-intelligence} 
%Based on a review of the literature, \cite{doshi-velezRigorousScienceInterpretable2017} identify a split in what is meant by ``interpretable.''
%Either a model is interpretable because it is useful to a human for some downstream task \citep[e.g.,][]{ribeiro2016should}, or a model is intuitively declared interpretable by nature of its construction \citep[e.g.,][]{lou2013accurate,rudin2019stop}.
%Both of these equate interpretability with explanation.
%Very little work to date has assessed the intrinsic interpretability of an algorithm, and those papers that do rely on user studies instead of analyzing the algorithm itself for properties that make it more or less interpretable.
%The study of algorithmic interpretability has not moved past intuition and downstream user-studies. 




%Customers and regulators still demand accountability in the form of an explainable decision-making process. 


\begin{comment} 
The field of explainable AI (xAI) has identified two ways to make sense of algorithms: studying the intrinsic interpretability of the algorithm itself and designing post-hoc explanability models to provide an explanation to users about a specific algorithmic decision. 
Post-hoc explanations are useful and correlate with user trust, performance, etc. \todo{(citations here)}. 
They link certain inputs to the output but are however independent of a study of the algorithm itself. 

The current state of research on intrinsic interpretability is intuition-driven, where certain classes of models (i.e., linear regression) are considered ``more interpretable'' than others (i.e., neural networks). 
To date intrinsic algorithmic interpretability has been understudied. 
Researchers focus on designing new post-hoc explanation methods and assessing them via downstream user studies. 
\todo{cites here, pull from earlier versions.}
There is a need for more quantified, rigorous research into intrinsic algorithmic interpretability \citep{leavitt2020towards}.
\end{comment}











\todo{Discuss. These are mostly what we did. We may want to summarize based on how these can be used.}
\begin{itemize}
    \item The proposed human-learning-based framework lays theoretical foundation for analyzing algorithmic interpretability. This work is an effort toward the call for developing formalized rigorous evaluation metrics \citep{Adadi2018}.
    \item The cognitive complexity score provides a quantifiable metric for IT managers to compare different candidate algorithms for a given task and balance the tradeoffs between algorithmic interpretability and other performance measures.
    \item The generated operation context graph offers a useful graphical representation of an algorithm for educational purposes.
\end{itemize}


This work contributes to research in algorithmic interpretability. 

\begin{itemize}
\item
  A \textit{framework for making sense of \frameworkname}~based on human expertise.
\item
An algorithm for converting any algorithm into a unique \graphname~graph
\item 
  \textit{\Graphname~graphs}, an enhanced graphical representation of an algorithm.
\item
  A \textit{cognitive complexity score} derived from the graph to quantify interpretability.
\end{itemize}




%%%%%%%%%%%%% COMMENTS %%%%%%%%%%%%%%

% below is text that has been commented out from earlier versions. we might want/need it moving forward so it's stored here. 


%As AI becomes more powerful and the algorithmization of the economy pushes forward \citep{lobel2020revenue}, users want to understand how AI affects them.
%Firms want to leverage algorithms and assess tradeoffs. 
%If an individual can interpret an algorithm and its outputs, then he or she can better reason about why certain outputs are generated. 

%Executives across industries recognize the potential of implementing algorithms into their processes, with 84\% of surveyed C-suite executives stating that they ``must leverage AI to achieve their growth objectives.''\footnote{https://www.accenture.com/us-en/insights/artificial-intelligence/ai-investments}


%These algorithms are black boxes, with little insight into how decisions are made. 
%Based on a review of the literature, \cite{doshi-velezRigorousScienceInterpretable2017} identify a split in what is meant by ``interpretable.''
%Either a model is interpretable because it is useful to a human for some downstream task \citep[e.g.,][]{ribeiro2016should}, or a model is intuitively declared interpretable by nature of its construction \citep[e.g.,][]{lou2013accurate,rudin2019stop}.


%
%Both of these equate interpretability with explanation.
%Very little work to date has assessed the intrinsic interpretability of an algorithm, and those papers that do rely on user studies instead of analyzing the algorithm itself for properties that make it more or less interpretable.
%The study of algorithmic interpretability has not moved past intuition and downstream user-studies. 
\begin{comment} 
As AI becomes more powerful and the algorithmization of the economy pushes forward \citep{lobel2020revenue}, users want to understand how AI affects them.
Regulators want to assess models for potential biases.\footnote{https://www.ftc.gov/news-events/blogs/business-blog/2021/04/aiming-truth-fairness-equity-your-companys-use-ai}\footnote{https://digital-strategy.ec.europa.eu/en/library/proposal-regulation-laying-down-harmonised-rules-artificial-intelligence-artificial-intelligence} 
Firms want to leverage algorithms and assess tradeoffs. 
Precise measurements for fairness, bias, and accountability are hard to define, so as a proxy researchers have turned to algorithm interpretability \cite{doshi-velezRigorousScienceInterpretable2017,lipton2018mythos}.
If an individual can interpret an algorithm and its outputs, then he or she can better reason about why certain outputs are generated. 

With the rise of big data and data-driven machine learning, algorithms are being applied to entirely new business domains.
Artificial intelligence (AI) and machine learning (ML) algorithms (hereafter ``algorithms'') are being deployed widely in industry.
Executives across industries recognize the potential of implementing algorithms into their processes, with 84\% of surveyed C-suite executives stating that they ``must leverage AI to achieve their growth objectives.''\footnote{https://www.accenture.com/us-en/insights/artificial-intelligence/ai-investments}
The benefits of implementing algorithms also come with risks.
These algorithms are not only being deployed to automate back-end business processes but are also being used in areas such as healthcare, criminal justice, and financial services.
They may exhibit biases when making predictions \citep{o2016weapons,kearns2019ethical,mehrabiSurveyBiasFairness2019}.



Executives struggle to implement AI models that they don't understand.
There is a consumer knowledge gap when it comes to AI.
Workers work around algorithmic management systems that they misunderstand. 
For AI and other technology innovations, workers are slower to adopt tech that they do not understand, costing firms money and productivity.
\end{comment} 

%Consider the question of identifying the largest number in a list. 
%Some function $f(x)$ will sort your list $x$ and return the largest value, $y$. 
%In post-hoc analysis, the question of why $y$ was returned will ignore the underlying algorithm. 
%Say $f(x)$ returns the first element in a list every time. 
%If the list is reverse-sorted it will return the correct answer, but not because the algorithm is correct. 
%An understanding of the algorithm itself is essential to allowing any kind of post-hoc explanation be deemed sufficient. 

%Intrinsic cognitive load can be characterized in terms of element interactivity \citep{MerrienboerSweller2005}.


%We propose a new research framework for \frameworkname.
%Our framework considers algorithmic complexity and user expertise as inputs to generate a novel graphical representation of algorithms. 
%From this graph we can calculate a cognitive complexity score, indicating how difficult it is for a user of a particular expertise level to understand the algorithm. 
%Our framework describes a user-specific, cognitive-load-centric, universal process for measuring the intrinsic interpretability of an algorithm.

%This work is orthoginal to the question of interpreting a \textit{specific decision} made by an algorithm.
%Instead we consider the algorithm itself, like the field of analysis of algorithms (CITE KNUTH BOOK). 

%This work applies to \textit{algorithms} in both the broad and narrow sense of the word.
%An algorithm is defined as ``a step-by-step procedure for solving a problem or accomplishing some end.'' (link to webster).
%For any algorithm a user either does or does not understand each ``step.''
%The steps are themselves algorithms that can be decomposed to step-by-step procedures. 
%Our framework enables the construction of graphical representations of algorithms at an appropriate level given domain knowledge. 


%How can we assess intrinsic algorithmic interpretability?


\begin{comment} 
To illustrate the current gap in algorithmic interpretability research and to preview to our framework consider the following story. 
In 1951 theoretical physicist Richard Feynman traveled to Brazil to teach physics.
He noticed that the students could memorize and recall definitions but had no understanding of underlying concepts \citep{feynman2018surely}: 

\begin{quoting}
\small 
  ``Triboluminescence. Triboluminescence is the light emitted when crystals are crushed…''

  I said, “And there, have you got science?
  No!
  You have only told what a word means in terms of other words \dots
  %You haven’t told anything about nature  what crystals produce light when you crush them, why they produce light.
  Did you see any student go home and try it?
  He can’t.

  But if, instead, you were to write, `When you take a lump of sugar and crush it with a pair of pliers in the dark, you can see a bluish flash.
  Some other crystals do that too.
  Nobody knows why.
  The phenomenon is called ``triboluminescence.'''
  Then someone will go home and try it.
  Then there’s an experience of nature.

\end{quoting}

To Feynman, the first definition of triboluminescence makes sense as he has internalized the necessary underlying concepts.
The students have not. 
Feynmam is describing his experience teaching physics in Brazil, but this captures the current state of explainable AI. 

Much of the work done today is ignoring the ``understandable'' piece of the definition provided above for interpretability.
Instead, xAI models generate explanations, humans look at them, and they think to themselves that they understand them.
Self-reported scores in research studies confirm this. 
But explanation doesn't equate with understanding if the explanation is not at an appropriate level. 
%Models themselves can be defined and explained in understandable terms, depending on an individual's level of expertise.
%To date no such method of interpretability exists.
%This is a significant gap in the literature. 
\end{comment} 



%We can measure how interpretable a particular AI or algorithm is.
%Each AI system is itself an algorithm, a recipe of steps to be executed one after another.
%Algorithms are by definition repeatable and consistent, and can be broken down into their operations.
%The operations can themselves be broken down further if needed.
%An operation to calculate an average can be decomposed to its addition and division operations.
%Similar to the emergence of analysis of algorithms, here we assume that very different algorithms share properties by nature of their construction as algorithms that make it possible to assess interpretability in a consistent way.
%Runtime complexity is an intrinsic property of an algorithm.
%The algorithm may run slower or faster on a specific computer.
%In a similar way the intrinsic interpretability of an algorithm can be measured.
%No such measure exists. 
%There is a gap in the literature around a quantified, cross-algorithm metric for measuring interpretability.


%A metric for algorithmic interpretability should consider both the human and computational elements of algorithms.
%Operations in an algorithm have a certain level of computational complexity, but the operations themselves may or may not be easy for a human observer to understand. 
%Algorithm complexity must be considered, but also some notion of cognitive complexity involved to understand the elements of the algorithm.
%Humans of different levels of ability will find algorithms more or less easy to understand based on their expertise. 
%The measurement should be universal, so that it can be applied to any algorithm, including complex machine learning models.
%Finally, the measurement itself and its construction should be easily understood so that firms can implement it when assessing tradeoffs.






\begin{comment} 
\todo{not sure about this motivating example}As a motivating example, consider the machine learning algorithm in Figure \ref{fig:tensorfloweg}.
This figure shows an example of a relatively simple learning algorithm implemented in TensorFlow, a popular machine learning library \citep{tensorflowPaper}.
Figures \ref{fig:1a} and \ref{fig:1b} show the code required to implement the algorithm using the TensorFlow Python application programming interface (API) and the corresponding computation graph, respectively (both from \cite{tensorflowPaper}). 
This algorithm could itself could be abstracted away and coded as a Python object which is then called in another program. 
This higher level abstraction would then look like Figure \ref{fig:1c} to those who are using the library.
All three representations in Figure \ref{fig:tensorfloweg} are equivalent, but they are not equally comprehensible for individuals with different backgrounds and domain knowledge. 
Any algorithm that can be programmed in TensorFlow (which includes deep neural networks as well as many other complex algorithms) can be represented by an equivalent computation graph.
\end{comment}



%\subsection{Framing} 


%Recent work has sought to set research agendas for algorithmic interpretability moving forward, either by focusing on building models that are inherently interpretable  or moving to a more rigorous research agenda for defining and evaluating interpretability based on post-hoc human evaluations \citep{DoshiKim2017Interpretability,abdul2018trends}.
%In this work we argue that there is a missing component: namely that each algorithm's intrinsic interpretability can be measured, and such a measurement is a key component of the algorithm.
%This work fits the latter call for more rigorous evaluation. 
%However in contrast to the taxonomy proposed in the prior work \citep{DoshiKim2017Interpretability}, \frameworkabbrv~\graphname~graphs allow for functionally-grounded evaluation (at the algorithm level) that depends on the acquired schemas of users.


